Voting based ensemble improves robustness of defensive models

Developing robust models against adversarial perturbations has been an active area of research and many algorithms have been proposed to train individual robust models. Taking these pretrained robust models, we aim to study whether it is possible to create an ensemble to further improve robustness. Several previous attempts tackled this problem by ensembling the soft-label prediction and have been proved vulnerable based on the latest attack methods. In this paper, we show that if the robust training loss is diverse enough, a simple hard-label based voting ensemble can boost the robust error over each individual model. Furthermore, given a pool of robust models, we develop a principled way to select which models to ensemble. Finally, to verify the improved robustness, we conduct extensive experiments to study how to attack a voting-based ensemble and develop several new white-box attacks. On CIFAR-10 dataset, by ensembling several state-of-the-art pre-trained defense models, our method can achieve a 59.8% robust accuracy, outperforming all the existing defensive models without using additional data.

==> rob_of_ensemble_defense.tex <==
\section{Robustness of Ensemble Defense} \label{rob-ens-def}
In this section, we will first introduce the proposed voting-based ensemble and provide empirical evidences showing it outperforms sum-of-logit based ensembles. Then we will discuss existing and newly proposed ways to attack voting-based ensemble in Section~\ref{attacks}. Finally, we discuss how to select the right subset of models to ensemble inSection~\ref{select-model-ens-0}. 
\subsection{Ensemble methods}
% \cho{Reorganize this subsection by the following paragraphs: 
% 1) Define the basic notations
% \\
% 2) Define sum-of-logit ensemble. Say many previous work use sum-of-logit ensemble but they don't work under straonger attack (talk about literature, and also maybe add some of our experiments
% \\
% 3) Define voting-based ensemble. (If we can, it will be good to explain why voting-based  ensemble work but not sum-of-logit ensemble. Maybe take a look at the cases where sum-of-logit fails but voting-based succeed and try to answer why voting-based ensemble is better)
% }
%\subsubsection{Notations}

We consider a $C$-way classification problem and assume there are $n$ neural network models that we want to ensemble. 
We denote an input as $(\mathbf{x}, y)$ where $\mathbf{x}\in \mathbb{R}^{d}$ is the input image and $y\in[C]$ is the class label.
The (logit layer) output of each neural network is defined by $f_i(\mathbf{x})\in \mathbb{R}^{C}$, and the hard-label decision of each network is denoted by 
\begin{equation*}
    F_i(\mathbf{x}) := \arg\max_{c=1, \dots, C} f_i(\mathbf{x})_c.
\end{equation*}

%Let there be $n$ neural networks with the $i^{th}$ network being a $C$ class $H_i$-layer feedforward classification neural network $f_i(\mathbf{x})\in \mathbb{R}^{C}$ as \devvrit{are these correct equations for wideresnet too?}
%\begin{align*}
    %f_i(\mathbf{x}) &= \mathbf{W}^{(H_i)}_{i}h_i^{(H_i-1)}(\mathbf{x}) + \mathbf{b}_i^{(H_i)}\\
    %h_i^{(l)}(\mathbf{x}) &= \sigma^{(l)}(\mathbf{W}_i^{(l)}h_i^{(l-1)}(\mathbf{x}) + \mathbf{b}_i^{(l)}), \forall l\in\{1,\cdots,H_i-1\}
%\end{align*}
%where $h_i^{(0)} = \mathbf{x}$, and layer $l$'s weight matrix for $i^{th}$ network is $\mathbf{W}_i^{(l)} \in \mathbb{R}^{n_l\times n_{l-1}}$ and bias vector is $\mathbf{b}_i^{(l)}\in \mathbb{R}^{n_l}$. Input $\mathbf{x}\in \mathbb{R}^{d}$ and we define $n_0=d$. $\sigma_i^{(l)}$ is a component wise activation function. We denote an input as $(\mathbf{x}, y)$ where $y\in[C]$ is the class label.

%\subsubsection{logits-summed ensemble} \label{logits-summed-ensemble}
\paragraph{Logits-summed ensemble}
Given $n$ networks in the ensemble, most of the previous methods use the \textit{logits-summed} ensemble \cho{cite}, where the decision function $f(\mathbf{x})$ is defined as 
%as a network with output $f(x) \in \mathbb{R}^{C}$ as
\begin{align*}
    f(\mathbf{x}) := \sum_{i=1}^{n}f_i(\mathbf{x}). 
\end{align*}
Informally, the logit output by the ensemble is basically the sum of logits by individual networks comprising the ensemble


%%%%%%%%%%%%%%%%%%%%%%%%%%
%inserting the table here 

\begin{table*}[h!]
\caption{Average $\cos(\theta)$ where $\theta$ is the angle between adversarial perturbation on pair of models under the same attack. Left (a) is on PGD-CE attack, right (b) is on C\&W attack \cho{Highlight the largest number in each row (I suppose diagonal elements are usually larger)}
\cho{Either mention what are defense 0, 1, 2, 3, 4 in the caption or write Trades/Mart/Trades+SAT/... explicitly in the table}
} \label{table0}
\centering

\begin{subtable}{.5\linewidth}
\caption{}
\centering

\begin{tabular}{|p{0.13\linewidth}|p{0.08\linewidth}|p{0.08\linewidth}|p{0.08\linewidth}|p{0.08\linewidth}|p{0.08\linewidth}|}
\hline
\textit{Defense} & \textit{0} & \textit{1} &\textit{2} &\textit{3} &\textit{4} \\
\hline
\textit{0} & 0.485 & 0.365 & 0.435 & 0.2 & 0.265\\
\textit{1} & 0.365 & 0.477 & 0.36 & 0.203 & 0.328\\
\textit{2} & 0.435 & 0.36 & 0.51 & 0.21 & 0.27\\
\textit{3} & 0.2 & 0.203 & 0.21 & 0.24 & 0.203\\
\textit{4} & 0.265 & 0.328 & 0.27 & 0.203 & 0.49\\
\hline
\end{tabular}
\end{subtable}%
\begin{subtable}{.5\linewidth}
\caption{}
\centering

\begin{tabular}{|p{0.13\linewidth}|p{0.08\linewidth}|p{0.08\linewidth}|p{0.08\linewidth}|p{0.08\linewidth}|p{0.08\linewidth}|}
\hline
\textit{Defense} & \textit{0} & \textit{1} &\textit{2} &\textit{3} &\textit{4} \\
\hline
\textit{0} & 0.39 & 0.287 & 0.343 & 0.16 & 0.276\\
\textit{1} & 0.287 & 0.395 & 0.28 & 0.179 & 0.313\\
\textit{2} & 0.343 & 0.28 & 0.41 & 0.167 & 0.26\\
\textit{3} & 0.16 & 0.179 & 0.167 & 0.197 & 0.176\\
\textit{4} & 0.276 & 0.313 & 0.26 & 0.176 & 0.408\\
\hline
\end{tabular}
\end{subtable}



\end{table*}



%%%%%%%%%%%%%%%%%%%%%%%%%%

%\subsubsection{majority-vote ensemble} \label{majority-vote-ensemble}
\cho{Unified the name of this. I think I called this ``voting-based ensemble'' in the intro, we should make the naming consistent. }
\paragraph{Majority-vote ensemble}
Given $n$ networks in the ensemble, we define the \textit{majority-vote} ensemble as a network with output $F(x) \in \mathbb{R}^{C}$ as
\begin{equation*}
    F(\mathbf{x}) := \arg\max_{c=1, \dots, C} \sum_{i=1}^n F_i(\mathbf{x}). 
\end{equation*}
%\begin{align*}
%    f(\mathbf{x}) &= e_{arg \ max(g(\mathbf{x}))}\\
%    \text{where } g(\mathbf{x}) &= \sum_{i=1}^{n}e_{arg \ max(f_i(\mathbf{x}))}
%\end{align*}
%where $e_{arg \ max(\mathbf{z})}$ is defined as an indicator vector with $1$ at the max component of vector $\mathbf{z}$ and $0$ otherwise. 
If more than one components have max value then assign $1$ to any one of them arbitrarily.
Informally, the majority-vote ensemble outputs a one-hot vector with prediction as the class having maximum vote by comprising individual networks in the ensemble.


\paragraph{Voting-based ensemble outperforms logits-summed ensemble.}
We found that the robust accuracy of logits-summed ensembles are often not much better than individual models. 
%We initially started with logits-summed ensemble, but got accuracies not much better than individual models. 
We believe this is mainly because logits-summed ensemble doesn't exploit the diverseness in decision boundaries as much as a voting based ensemble does. We considered the following $5$ recently proposed state-of-the-art defenses: Trades \cite{zhang2019theoretically}, Mart \cite{Wang2020Improving}, TRADES+SAT \cite{huang2020selfadaptive}, ATES \cite{sitawarin2020improving}, and PGD+HE \cite{pang2020boosting}. We chose these particular defenses as they have very similar performance---their robust accuracies are within $0.7\%$ of each other (Table \ref{table4}). We form ensemble of $3$ models, hence $5^3=125$ possibilities. \cho{Reviewers might confuse why can we ensemble the same model. We need to make it clear that we can ensemble the same model with different initialization points. } Testing these many ensembles is tough, hence we tested a big and good representative subset of them. For logits-summed ensemble, we tested all possible ${5\choose3}=10$ ensembles consisting three models all of different defense method, $7$ ensembles consisting $2$ models of one defense type and $1$ of some other defense type, and $3$ ensembles consisting all three models of same defense type. The highest accuracy against LA-Autoattack \cho{don't use math font for this, please try to correct other places}\devvrit{Will do, sorry about that}, the strongest defense against logits-summed ensemble (introduced later), is $57.9\%$. Whereas the highest accuracy using the same set of models but with voting-based ensemble, under WA-autoattack (strongest attack for voting based ensemble, introduced later), was $59.17\%$ -- got from just testing ${5 \choose 3}=10$ ensembles consisting three models all of different defense type.\\
The advantage of voting-based ensemble becomes even more stark when we add a weaker but possibly more diverse model to our pool of individual models. We considered PGD \cite{madry2017towards} model in addition to above $5$ models, though PGD has much lower accuracy (Table \ref{table4}). While voting-based ensemble accuracy increased to $59.2\%$, there wasn't any gain for logits-summed ensemble \cho{but 59.2 is only slightly better than 59.17 without PGD? Also, need to give exact numbers for logits-summed ensembles.} \devvrit{PGD is also way less robust so maybe that could be a reason. Also, there's another variant of PGD called PGD+HE that we use in the previous set of 5 models. Hence maybe that already captures the diverseness of PGD somewhat. Not sure of exact reasons}. In fact, to the contrary, any logits-summed ensemble consisting PGD model performed poorly ($<54\%$ accuracy). Upon inspection, we found that most of the points were able to fool just the PGD model, but this one fooled model drove sum of logits to predict the wrong class. \\

\cho{Instead of giving the numbers in paragraph, it's better to draw some tables or figures. We can have one figure (maybe bar chart?) for comparing voting based vs logit-sumed ensemble. }
\devvrit{Sure, I'll work on this section soon.}





% Consider as an example a $3$ class classification instance where we're given three models, say, $A,B,$ and $C$. Suppose $A$ is robust on class-1 and class-2 but not on class-3. Whereas $B$ is robust on class-2, class-3, but not on class-1. And $C$ is robust on class-1, class-3, but not on class-2. In this case, a voting based ensemble would surely lead to robustness over every class because each class is robust with respect to $2$ out of the $3$ models. However, a logits-summed ensemble could possible perform bad here if the model which is non-robust on a given class drives sum of logits towards the wrong class


% For example, in the case of [PGD, Mart, Trades], the LS-CE attack (introduced later) got 51.9\% accuracy on the logits-summed ensemble. In order to investigate the reason for low accuracy, we calculated the individual robust accuracy on each of the Trades, Mart, and PGD model on the adversarial points generated for this logits-summed ensemble. We found that accuracy of Trades and Mart was high - 65.5\% and 66.8\% respectively, but of PGD was low - 48.8\%. This means that PGD model logits were driving the sum of the logits towards the wrong class. In fact, if we rather attack the [PGD, Mart, Trades] logits-summed ensemble but measure the final accuracy by just taking sum of logits of Mart and Trades without including PGD, the accuracy comes around 66.19\%.
% using the same adversarial points against against sum of logits of just Trades and Mart gave 66.19\% accuracy. That is, we took the same setting of [PGD, Mart, Trades] ensemble, performed LS-CE attack on it, but while measuring the final accuracy rather than measuring it on sum of logits of Trades, Mart, and PGD, measured only on sum of logits of Trades and Mart to get 66.19\% accuracy.
% This clearly indicates that PGD model logits drove the sum of logits to predict the wrong class.\\

% \noindent Previous work are mostly logits-summed based and trained on same loss function. Moreo Hence we decide to 
% As two of the three models were still predicting correct for most of the points, we rather decided to use majority-vote ensemble.

\noindent To illustrate why voting-based ensemble can improve robustness, we measure the diverseness of decision boundaries due to the loss functions they are trained on, for several pairs of models. We took pairs of models, attacked them individually with the same attack (say, PGD attack with CE loss), and measured the average cosine of angle between perturbations generated for the pair of models. We'd expect that if indeed models trained on different loss functions are more diverse, their adversarial perturbations will be more diverse too (hence smaller $\cos(\theta)$) compared to a pair of models which are trained on the same loss function (hence larger $\cos(\theta)$). We took $5$ recently proposed state-of-the art defenses\footnote{we would have taken more but could find training code available for only 5 of them}: Trades \cite{zhang2019theoretically}, Mart \cite{Wang2020Improving}, Trades-AWP \cite{wu2020adversarial}, PGD \cite{madry2017towards}, and PGD+HE \cite{pang2020boosting}. We denote them as $0,1,2,3,4$ respectively in Table \ref{table0} for brevity. We trained $2$ models of each defense method, attacked them using PGD attack and C\&W attack \cite{Carlini_2017}, and measured average $\cos(\theta)$ of the perturbations for all $5*5=25$ pairs of models. Here, $\theta$ represents the angle between perturbation generated for a given point $\textbf{x}$ by an attack on the pair of models under consideration. We report the number in Table \ref{table0} and notice that the angle between two models of same defense type is consistently smaller than the angle between two models trained on different loss functions. We believe this is some metric, if not the perfect metric, to show the difference in diverseness of decision boundary of pairs of models trained on the same loss function compared to different loss functions.\\
Note that a voting-based ensemble would be able to make good advantage of diverseness in decision boundary, compared to a logits-summed ensemble. Consider as an example a $3$ class classification instance where we're also given three models, say, $A,B,$ and $C$. Suppose $A$ is robust on class-1, class-2 but not on class-3. Whereas $B$ is robust on class-2, class-3, but not on class-1. And $C$ is robust on class-1, class-3, but not on class-2. In this case, a voting based ensemble would surely lead to robustness over every class because each class is robust with respect to $2$ out of the $3$ models. However, a logits-summed ensemble could possible perform bad here if the model which is non-robust on a given class drives sum of logits towards the wrong class, as we saw when we took PGD model with other defense type models to form logits-summed ensemble.

% We initially started with \textit{sum-of-logits} ensemble but observed it performes poorly. Upon inspection we found that most of the points were able to fool just one of the three models, but that one fooled model was quite sure about the wrong label, driving sum of logits to predict the wrong class. As two of the three models were still predicting correct in this case, we rather decided to use \textit{majority-vote} ensemble.

\subsection{Model Selection  for voting-based ensemble} \label{select-model-ens-0}
Given $n$ individual defenses, our aim is to select $k$ defenses out of the $n$ available to form a voting-based ensemble. This problem isn't easy to solve as it requires selecting models based on how individually robust they are, as well as how diverse they are with respect to each other. In the following, we model this problem from an optimization point of view and derive an algorithm for model selection. 


 Let $\{f_1(\mathbf{x}),f_2(\mathbf{x}),\cdots,f_{n\choose k}(\mathbf{x})\}$ be the possible ${n\choose k}$ ensembles formed of $k$ models each, where $f_i(\mathbf{x})\in \mathbbm{R}^{C}$. Consider the distribution of domain to be $D$. That is, $(\mathbf{x},y)\sim D$ such that $y\in [C]$.
% Consider $r$ points $\{\mathbf{x_1},\cdots,\mathbf{x_r}\}$ with true labels $\{y_1,\cdots,y_r\}$ where $y_i\in [C]$. 
Let the set of allowed perturbations belong to set $\mathcal{B}$. For example, $\mathcal{B}= \epsilon$ sized $l_{p}$ ball is one of the perturbations used in practice. Let $\mathbf{x_i'}$ be a valid perturbation for point $\mathbf{x_i}$ if $(\mathbf{x_i'}- \mathbf{x_i}) \in \mathcal{B}$.
% Let $\{\mathbf{x_1'},\cdots,\mathbf{x_r'}\}$ be perturbed point corresponding to $\{\mathbf{x_1},\cdots,\mathbf{x_r}\}$ such that $(\mathbf{x_i'}- \mathbf{x_i}) \in \mathcal{B}$.
Let $sc(f_i, \mathcal{B}, D)$ denote the score of $i^{th}$ ensemble defined as $sc(f_i, \mathcal{B}, D) = \underset{(\mathbf{x},y)\sim D}{\mathbb{E}}[\mathbbm{1}_{f(\mathbf{x'})=y}]$ where $\mathbf{x'}$ is a valid perturbation of point $\mathbf{x}$ and $y$ is the corresponding label. Then, the optimization problem for ensembles basically becomes:
\begin{align}
    \underset{i}{max} \ \underset{\delta \in \mathcal{B}}{min} \ sc(f_i, \mathcal{B}, D) \label{eq:choosing-ensemble}
\end{align}
Intuitively, the optimization problems considers all possible ensembles, calculates their worst perturbation and hence an absolute measure of their robustness, and asks to choose the best ensemble among all possible.
This is similar to \citet{madry2017towards} min-max objective, but different for other reasons. Note that \citet{madry2017towards} min-max objective is intractable even if given the entire distribution $D$, as it asks to consider all possible decision boundaries of the model. However, because the ensembles are fixed here, given a distribution $D$, the problem is tractable by iterating over the set of possible ensembles and measuring their robustness.\\
When not given the distribution itself, we solve an ERM version of eq.\ref{eq:choosing-ensemble}. There are two other two 1) considering ${n\choose k}$ ensembles, which could be pretty large depending on $k$; 2) finding best perturbation for each ensemble. The first could be addressed by using some combinatorial optimization techniques like genetic algorithm ({\color{red} citation?}) to approximate the best ensemble. Though, when $k$ is small, one could do a brute force enumeration. The second problem is tough to answer as it requires testing ensembles which is costly. Also, there isn't one perfect metric to generate the most optimal perturbations.\\
Hence, we use a heuristic to approximate the eq.\ref{eq:choosing-ensemble} objective. We take $r$ random test/validation points $\{\mathbf{x_1},\cdots,\mathbf{x_r}\}$ with true labels $\{y_1,\cdots,y_r\}$ where $y_i\in [C]$. We generate perturbation for each point by attacking any one of the $n$ models. To maintain uniformity, we use the first model to generate perturbations for the first $r/n$ points, the second model for next $r/n$ points, and so on. Then for each ${n \choose k}$ possible ensembles, we calculate its score as the number of adversarial points predicted corrected by at least $\lceil k/2 \rceil$ out of the $k$ models in the ensemble. This is because we're focusing on voting-based ensemble and so using its definition to calculate the ensemble's score. Finally, we choose the ensemble with the highest score.\\
Intuitively, testing a model on adversarial points captures the model's robustness. And testing the adversarial points generated by one model on another tests transferability and hence the diverseness of different models with respect to each other. We later show this heuristic gives a reasonable approximation to the actual eq.\ref{eq:choosing-ensemble} objective in Section \ref{select-model-ens}, by considering a pool of $7$ different defenses.

\subsection{Attacks} \label{attacks}
As we want to objectively test the robustness, we perform white-box attacks on all the ensembles. There hasn't been \textbf{any} systematic study on developing white-box attacks to test majority-vote ensemble. Here, we propose four different attack techniques which could be used on top of any existing white-box attacks to test voting-based ensemble.
\subsubsection{Logits-summed attack} \label{LS}
The attacker has access to all the weight and the architecture of the individual models used in the ensemble. The attacker takes logits of all the individual models, sums them up and perform a white-box attack against this set of logits.
% That is, the attacker attacks logits-summed ensemble irrespective even if the ensemble used is majority-vote ensemble.
This attack technique was also used in \cite{tramer2020adaptive} against \cite{sen2020empir}.

Note that this technique gives us freedom to use any white-box based attack against sum of the logits. We use PGD with CE loss attack (\cite{aleks2017deep}), FAB-attack (\cite{croce2019minimally}), and autoattack (\cite{croce2020reliable}) using this technique to test ensemble robustness.

\subsubsection{Weakest-attacked attack} \label{WA}
Let the point in consideration be $(\mathbf{x},y)$. Let there be $n$ networks in the ensemble. The attacker calculates logits $f_i(\mathbf{x})$ for all $n$ networks. If the majority vote $f(x)$ for majority-vote ensemble (as defined in Section \ref{majority-vote-ensemble}) is already the non-true class, then the attacker is done. Otherwise, among the individual models (also referred to networks in this work) which predict correct label $y$, the attacker chooses the weakest model and performs a local small step attack on it. The weakest model among those which predict the true class $y$ is determined by calculating the probability of individual models on true class $y$ and choose the one with lowest probability. Let $\mathbf{y} \in \mathbb{R}^{C}$ represent the one-hot vector with $1$ at component $y$ and 0 otherwise. Mathematicaly the weakest model output can be represented as $f_{k}(\mathbf{x})$ where
\begin{align*}
    k &= \underset{i\in [n]}{arg \ min} \  (\mathbbm{1}_{f_i(\mathbf{x})=\mathbf{y}}\cdot (p_i(\mathbf{x}))_{y} + \mathbbm{1}_{f_i(\mathbf{x})\neq \mathbf{y}}\cdot 1)\\
    &\text{where } p_i(\mathbf{x}) = Softmax(f_i(\mathbf{x}))
\end{align*}
where $\mathbbm{1}$ is an indicator variable and $(p_i(\mathbf{x}))_{y}$ refer to the $y^{th}$ component of vector $p_i(\mathbf{x})$.

Take an example of an ensemble consisting of three models $\{m_1,m_2,m_3\}$. Let the clean data point be $x$ and its true class be $y$. The attacker checks if the majority vote is already a non-true class. If so, the attacker is done. Let's say this is not the case and $\{m_1,m_2\}$ predict the true class $y$. Also let the probability of class $y$ predicted by $m_1$ be less than that predicted by $m_2$. Most of the existing white-box based attacks happen by taking multiple small steps towards final perturbation. In this case, the attacker performs a local attack on $m_1$ and moves $x$ to $x+\epsilon$. The attacker again passes this $x+\epsilon$ through all three models $\{m_1,m_2,m_3\}$. Let's say still $\{m_1,m_2\}$ predict the true class $y$ but this time probability of class $y$ by $m_2$ is less than that of $m_1$. In this step, the attacker performs a local attack on $m_2$ to to get $x+\epsilon+\epsilon'$. This is repeated until either the number of steps are over or the majority vote becomes a non-true class. Intuitively, the attacker performs a greedy attack over the three models to turn the majority vote to a non-true class.

Note that similar to logits-summed attack technique, this attack technique could also use any existing white-box attack. We never fixed what attack is applied on the locally weakest model. In this work we consider PGD with CE loss attack(\cite{aleks2017deep}), FAB-attack (\cite{croce2019minimally}), autoattack (\cite{croce2020reliable}), and $l_{\infty}$ B\&B attack (\cite{brendel2019accurate}) with this attack technique.

\subsubsection{Objective-summed attack} \label{CW}
% \cho{I feel this can be more general? For any attack (e.g., PGD) we can sum the objective and conduct this attack. We can say this is a general attack (like the previous two) and we try to use C\&W in practice. }
Most of the existing white-box attacks decrease/increase a particular objective. For example, PGD attack with CE loss function maximizes the CE loss, C\&W attack minimizes the C\&W loss (\cite{Carlini_2017}). Therefore another attack technique is to take sum of this attack objective values on individual models of the ensemble and decrease/increase it. Notice that just like previous techniques, even this method can work with any white-box attack. In this work, we particular consider C\&W loss objective. That is, we sum the C\&W loss over all the models comprising the ensemble, and decrease it using PGD.

% For  given single model with output $f_i(\mathbf{x}) \in \mathbb{R}^{C}$ and an input $(\mathbf{x},y)$, \citet{Carlini_2017} introduced an attack aimed at optimizing the following function
% \begin{align*}
%     l_i(\mathbf{x}) = max((f_i(\mathbf{x}))_y - (f_i(\mathbf{x}))_{y'}, -\kappa)
% \end{align*}
% where $(f_i(\mathbf{x}))_y$ is the $y^{th}$ component of $f_i(\mathbf{x})$ and $y'$ is the class having highest logit among all classes except $y$. Therefore, $(f_i(\mathbf{x}))_{y'}$ is the highest logit among non-true class. $\kappa$ is a hyperparameter denoting how strongly we want the classifier to output the wrong class.

% Let there be $n$ individual models in the ensemble represented by $\{m_1,\cdots,m_n\}$. Let $l_i(\mathbf{x})$ denote the C\&W loss on the $i^{th}$ model. Then, the attacker optimizes upon $L(\mathbf{x}) = \sum_{i=1}^{n}l_i(\mathbf{x})$. We test all the ensembles against this paritcular attack, calling it simply C\&W attack.
\subsubsection{majority-attack}
Rather than using the previous three introduced attack technique over the entire ensemble, one can use them over just a subset of $\lceil n/2 \rceil$ models among the $n$ models comprising the ensemble. Intuitively, as voting-based ensemble needs to misclassify any $\lceil n/2 \rceil$ models, the attacker focuses on doing just that. One needs to consider all possible ${n \choose n/2}$ combination though, hence this attack technique isn't very efficient. But for small $n$ one can use it. In this work, we use Objective-summed attack technique (Section \ref{CW}) with C\&W attack on an ensemble consisting $3$ models and attack all possible ${3 \choose 2}$ pairs of models of the ensemble.

% Let $S$ be a subset containing $\lceil n/2 \rceil$ models among the $n$ models of the ensemble. Then, rather than optimizing over sum of objectives over all the models as proposed above, the attacker optimizes over sum of objective only on the models in this set $S$ and taking the best attack over all possible subsets $S$. For C\&W attack, this translates to optimizing over $L(\mathbf{x}) = \sum_{i\in S}l_i(\mathbf{x})$ and taking the best attack over all the possible subsets $S$. Intuitively, as voting-based ensemble needs to misclassify any $\lceil n/2 \rceil$ models, the attacker focuses on doing just that.
% The other closely related attack is when attacker optimizes upon $F(x) = \underset{i}{max} \ f^{(i)}(x)$.

% We noticed during our experiments that either logits-summed attach technique or weakest-attacked attack technique works better than any of the above two C\&W attacks. Therefore, we only report our experiments on these two attack techniques and not on C\&W based attack


% \mh{it is weird to have a section called notations here if it is about the experiments. You could list it as a subsection like CAT paper. like "implementation details" etc.}

% \cho{I think we can have another version of this. For example, if there are models $m_1, m_2, m_3$, ideally we can try to attack each 2 models. For attacking each 2 models we can use sum of their C\&W loss function as objective to run the attack (so instead of attacking sum of three C\&W loss as you did here, try to attack sum of two C\&W loss and try all the three combinations and select the best. }

% \subsection{Choosing individual models}
% One of the main objective in this work is to show that pretrained models trained on diverse losses form a good ensemble because the different losses encourage diverse decision boundary. Unfortunately, we don't have a perfect metric to capture the "difference" in loss function. Hence, we use a few recently proposed pre-trained model which don't train on the exact same loss function. We use our intuition to judge the "difference" in loss function. For example, consider Trades with different $1/\lambda (\text{or }\beta)$ parameters. Intuitively, the structure of the loss function is same with the difference being in just one parameter. Hence, this "difference" in loss functions between various Trades loss functions with different $1/\lambda$ seems less than, say, between PGD loss function (\cite{aleks2017deep}) and Trades loss function (\cite{DBLP:journals/corr/abs-1901-08573}). The PGD min-max loss function minimizes loss considering perturbation in the worst case. Whereas Trades looks at the clean accuracy along with another term capturing how much robustness we want to force. Having a metric to capture the "difference" in loss function is an interesting topic we leave as future work.
